LeapFrog: The Rowhammer Instruction Skip Attack

Since its inception, Rowhammer exploits have rapidly evolved into increasingly sophisticated threats compromising data integrity and the control flow integrity of victim processes. Nevertheless, it remains a challenge for an attacker to identify vulnerable targets (i.e., Rowhammer gadgets), understand the outcome of the attempted fault, and formulate an attack that yields useful results. In this paper, we present a new type of Rowhammer gadget, called a LeapFrog gadget, which, when present in the victim code, allows an adversary to subvert code execution to bypass a critical piece of code (e.g., authentication check logic, encryption rounds, padding in security protocols). The LeapFrog gadget manifests when the victim code stores the Program Counter (PC) value in the user or kernel stack (e.g., a return address during a function call) which, when tampered with, repositions the return address to a location that bypasses a security-critical code pattern. This research also presents a systematic process to identify LeapFrog gadgets. This methodology enables the automated detection of susceptible targets and the determination of optimal attack parameters. We first show the attack on a decision tree algorithm to show the potential implications. Secondly, we employ the attack on OpenSSL to bypass the encryption and reveal the plaintext. We then use our tools to scan the Open Quantum Safe library and report on the number of LeapFrog gadgets in the code. Lastly, we demonstrate this new attack vector through a practical demonstration in a client/server TLS handshake scenario, successfully inducing an instruction skip in a client application. Our findings extend the impact of Rowhammer attacks on control flow and contribute to developing more robust defenses against these increasingly sophisticated threats.

==> TODOs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%    IN PROGRESS    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
## IN PROGRESS | Add some experiments with performance degradation to achieve synchronization in a realistic way. This will definitely be asked by the reviewers. - andrew
    - -> hyperdegrade - Shared library cache attack for synchronization

%%%%%%%%%%%%%%%%%%%%%%%   TODO    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
## look at the Rowhammer countermeasure, show they don't apply into our attack. - andrew
    - pointer authentication
    - mL based mitigation
    - uarch change

## Ideas from the meeting on 12/23/2022 
-> Separate online and offline phase to reduce crashing - This may not help
-> Experiment with huge pages (this may solve crashing and may find more flips)
-> Find most common relaunch bait page value
-> Experiment by mmaping after a relaunch and ensuring that the flippy page is released...

%%%%%%%%%%%%%%%%%%%%%%% WRITING TODO  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
## sudo attack would be classified as "LPE (Local Privilege Escalation) exploit" by the hacker community. we should use the term in the paper.

## explain how we solved system crashes - say you're speculating
    - my guess is it's flipping far away bits outside our attack window. MARGIN does not solve reliably because our continuous window is not actually fully continuous.
    - we need to add the margin for every continuous chunk in every bank.

## add timing side-channel for aslr leak as a negative result.

## explain the syncronization vs performance degradation. we don't need anything extra for syncronization in sudo and SSH attacks. performance degradation is only for making sure the variable stays long enough in the memory for Rowhammer.

## explain we don't need sudo in the target system to determine the # bait pages.

## explaing why existing performance degradation techniques do not work well enough. > because the target window is so small. so effect is small.

%%%%%%%%%%%%%%%%%%%%%%% LEFT FOR THE FUTURE WORK  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
## find an authentication flag in PAM libraries - caner

## Write a script to automate finding authentication flags - caner
    - brute force is not easy because we can even target the registers. it needs a more sophisticated method.
    
## Figure out breaking stack ASLR - caner
- we added page faults graph - done 
- try sched\_yield() for remapping
- collect HPC data together with page offsets to see which component is affected.

%%%%%%%%%%%%%%%%%%%%%%%     DONE    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
## DONE | Try sched_yield for improving bait page success
        - no significant effect

## DONE | Keep the flippy page and relaunch sudo (we expect that it will come back to the same flippy page, but may come to the same flippy page)
	-> Use sudo, but without rowhammer
        - does not work very well but explained in the text.
        
## DONE |  Keep ASLR off and increase 43\% to 100\% bait page (figuring this out may improve our ASLR enabled bait page technique) 
	-> What's different between rowhammer and attack_stack
 
## DONE | run rowhammer on OPENSSL and get offline time, online time, success rates - andrew

## DONE | Examine crypto libraries for potential targets - yarkin, berk
    - RSA BELLCORE is examined in openssl. other don't work.
    
## DONE | run rowhammer on SSH and  get offline time, online time, success rates - caner
    - roadblock: python code gets stuck at readline() (SOLVED)
    - ran for 2 days 16\% successful baits, no offset aligned no flips
    
## DONE | Install MySQL and find authentication flags that we can flip. Other options: MySQL, PostgreSQL, MariaDB, Oracle Database, and Microsoft SQL Server - caner
    - Installed MySQL, now looking for working flags.
    - problem: rebuilding takes too long to try different flags
    - trying to build it on flash server
    - "make mysqld" takes less time, around 1.5 minutes. also, don't run cmake after each change.
    
## DONE | run DDR4 rowhammer on SUDO and get offline time, online time, and success rates - andrew
    - logging problem got solved. now running the experiment.
    - python script sometimes gets stuck at the readline() 
    - 2 offset aligned but no flips.
    - we saw 1 flip.
    
## DONE | Generate heatmap for DDR4 - caner
    problem: the OS keeps crashing. I need more time with the machine. 
    - make margin 200 and try again. * it worked fine with zero margin 8MB for 3 days.
    - forgot to include page offset in physical addresses. 
    running the experiment again.
    
## DONE | Fix signals in SUDO attack- Workaround: Put sleep(3)- andrew

## DONE | fix signals with OpenSSH - caner

## DONE| generate Bait and Page offset graphs for SSH attack - caner
    problem: about 75\% -1's. about 10-15\% goes to a nonzero bait page.
    - will try running the client from another machine.
    - the reason was server was running on another core and client in the isolated core. Now I co-locate server and attacker on the same core and run client on another core. It's become very stable.

## DONE | run SUDO attack after setting matched=1 and check the log file and python code output. - andrew/caner
    - it will not hang in the root anymore but it will print Flipped into the log file and continue the attack instead.

## DONE | run SUDO attack from the console mode of Ubuntu to reduce the noise coming from GUI. - andrew

## DONE |  Send email about huge pages to Graz team - caner
    - I've sent an email to Tian Guo from WPI CS department. She teaches OS.
    
## DONE | run SUDO attack after adding sched\_yield()  - andrew
    - it doesn't really help.
